Bilinear Generalized Vector Approximate Message Passing

We introduce the bilinear generalized vector approximate message passing (BiG-VAMP) algorithm which jointly recovers two matrices U and V from their noisy product through a probabilistic observation model. BiG-VAMP provides computationally efficient approximate implementations of both max-sum and sumproduct loopy belief propagation (BP). We show how the proposed BiG-VAMP algorithm recovers different types of structured matrices and overcomes the fundamental limitations of other state-of-the-art approaches to the bilinear recovery problem, such as BiG-AMP, BAd-VAMP and LowRAMP. In essence, BiG-VAMP applies to a broader class of practical applications which involve a general form of structured matrices. For the sake of theoretical performance prediction, we also conduct a state evolution (SE) analysis of the proposed algorithm and show its consistency with the asymptotic empirical mean-squared error (MSE). Numerical results on various applications such as matrix factorization, dictionary learning, and matrix completion demonstrate unambiguously the effectiveness of the proposed BiG-VAMP algorithm and its superiority over stateof-the-art algorithms. Using the developed SE framework, we also examine (as one example) the phase transition diagrams of the matrix completion problem, thereby unveiling a low detectability region corresponding to the low signal-to-noise ratio (SNR) regime.

==> figure3.tex <==
\begin{tikzpicture}[thick,scale=1.0, every node/.style={scale=1.0}]
  % Define nodes
  % U nodes
  \node[latent]  (ui2)   {$\textrm{\textbf{{\rv{u}}}}_{i}^-$};
  \node[latent, xshift=-3cm, yshift=0cm]  (ui1)   {$\textrm{\textbf{{\rv{u}}}}_{i}^+$};
  % V nodes
  %\node[latent, xshift=-2cm]  (vj1)   {$\boldsymbol{v}_{1,j}$};
  \node[latent, right=of ui2, xshift=0cm]  (vj2)   {$\textrm{\textbf{{\rv{v}}}}_{j}^-$};
  \node[latent,  xshift=5.05cm, yshift=1.5cm]  (vj1)   {$\textrm{\textbf{{\rv{v}}}}_{j}^+$};
  %
  % Y node
  %\node[latent, above=of fij, xshift=1.75cm, yshift=1.4cm, fill=light-gray]  (yij)   {$y_{ij}$};
  %
  \node[latent, above=of fij, xshift=3.75cm, yshift=1.4cm, fill=light-gray]  (yij)   {$\bm{\mathsf{Y}}$};
  %
  % Factor node fij: I use \scalebox to resize its text
  \factor[right=of ui2, xshift=0.75cm, xscale=2.5, yscale=2.5] {fij}  {below:  \scalebox{0.8}{ $ p_{\textrm{{\rv{Y}}} | \textrm{\textbf{{\rv{U}}}}^-\!,\, \textrm{\textbf{{\rv{V}}}}^-}(\bm{Y} | \bm{U}^-, \bm{V}^-;\gamma_w)$}
  } {ui2, vj2, yij}{};
  
  % Equality Factor node ui2==ui1
  \factor[left=of ui2, xshift=-0.5cm,xscale=2.5, yscale=2.5] {eq_ui1_ui2}  {below: $\delta(\boldsymbol{u}_{i}^- - \boldsymbol{u}_{i}^+)$ } {ui2, ui1}{};
  
  % Equality Factor node vj2==vj1
  \factor[right=of vj2, xshift=0.5cm, xscale=2.5, yscale=2.5] {eq_vj1_vj2}  {below:  $\delta(\boldsymbol{v}_{j}^- - \boldsymbol{v}_{j}^+)$} {vj2, vj1}{};
  
  % Prior factor node of U
  \factor[left=of ui1, xscale=2.5, yscale=2.5] {pui1} {left:$p_{\textrm{\textbf{{\rv{u}}}}_{i}^+}(\cdot)$} {ui1} {};
  
  % Prior factor node of V
  \factor[above=of vj1, xscale=2.5, yscale=2.5] {pvj1} {right:$p_{\textrm{\textbf{{\rv{v}}}}_{j}^+}(\cdot)$} {vj1} {};

  % message from fij to vj
  \node (f_v2_right) at ($(vj2)!0.5!(fij) + (-0.25,0.5)$) {};
  \node (f_v2_left) at ($(vj2)!0.5!(fij) + (0.25,0.5)$) {};
  %\draw [-latex,very thick] (f_v2_right.center) -- (f_v2_left.center);
  %\node[right=of f_v2_left, xshift=-1.22cm, yshift=0.025cm] (id_f_v2) {\protect\tikz[inner sep=.25ex,baseline=-.75ex] \protect\node[circle,draw] {{\tiny 2}};};

  % message from fij to vj
  \node (v2_f_right) at ($(vj2)!0.5!(fij) + (0.1,0.25)$) {};
  \node (v2_f_left) at ($(vj2)!0.5!(fij) + (-0.4,0.25)$) {};
  \draw [-latex,very thick] (v2_f_left.center) -- (v2_f_right.center);
  \node[right=of f_v2_right, xshift=-0.87cm, yshift=-0.25cm] (id_v2_f) {\protect\tikz[inner sep=.25ex,baseline=-.75ex] \protect\node[circle,draw] {{\tiny 2}};};
  
  % message from fij to uj2
  \node (f_u2_right) at ($(ui2)!0.5!(fij) + (0.4,0.25)$) {};
  \node (f_u2_left) at ($(ui2)!0.5!(fij) + (-0.1,0.25)$) {};
  \draw [-latex,very thick] (f_u2_right.center) -- (f_u2_left.center);
  \node[left=of f_u2_left, xshift=0.5cm, yshift=0.25cm] (id_f_u2) {\protect\tikz[inner sep=.25ex,baseline=-.75ex] \protect\node[circle,draw] {{\tiny 1}};};
  
  % message from uj2 to fij
  \node (u2_f_right) at ($(ui2)!0.5!(fij) + (0.4,0.5)$) {};
  \node (u2_f_left) at ($(ui2)!0.5!(fij) + (-0.1,0.5)$) {};
  %\draw [-latex,very thick] (u2_f_left.center) -- (u2_f_right.center);
  %\node[left=of f_u2_left, xshift=2.1cm, yshift=0.25cm] (id_u2_f) {\protect\tikz[inner sep=.25ex,baseline=-.75ex] \protect\node[circle,draw] {{\tiny 3}};};
  
  % message from delta to ui1
  %\node (d_u1_top) at ($(ui1)!0.5!(eq_ui1_ui2) + (-0.5,0.1)$) {};
  %\node (d_u1_bottom) at ($(ui1)!0.5!(eq_ui1_ui2) + (-0.5,-0.4)$) {};
  %\draw [-latex,very thick] (d_u1_bottom.center) -- (d_u1_top.center);
  %\node[above=of d_u1_top, xshift=0cm, yshift=-1.35cm] (id_d_u1) {\protect\tikz[inner sep=.25ex,baseline=-.75ex] \protect\node[circle,draw] {{\tiny 1'}};};fuck
   \node (f_u2_right) at ($(ui2)!0.5!(eq_ui1_ui2) + (0.2,0.25)$) {};
  \node (f_u2_left) at ($(ui2)!0.5!(eq_ui1_ui2) + (-0.3,0.25)$) {};
  \draw [-latex,very thick] (f_u2_right.center) -- (f_u2_left.center);
  \node[above=of f_u2_left, xshift=0.25cm, yshift=-1.2cm] (id_f_u2) {\protect\tikz[inner sep=.25ex,baseline=-.75ex] \protect\node[circle,draw] {{\tiny 1'}};};
  
  % message from vj1 to delta
  \node (u1_d_top) at ($(ui1)!0.5!(eq_ui1_ui2) + (-0.25,0.3)$) {};
  \node (u1_d_bottom) at ($(ui1)!0.5!(eq_ui1_ui2) + (-0.25,-0.3)$) {};
  \draw [-latex,very thick] (u1_d_top.center) -- (u1_d_bottom.center);
  \node[below=of u1_d_bottom, xshift=-0.3cm, yshift=1.75cm] (id_u1_d) {\protect\tikz[inner sep=.25ex,baseline=-.75ex] \protect\node[circle,draw] {{\tiny 3'}};};
  
  % message from delta to vj1
  %\node (d_v1_top) at ($(vj1)!0.5!(eq_vj1_vj2) + (0.5,0.1)$) {};
  %\node (d_v1_bottom) at ($(vj1)!0.5!(eq_vj1_vj2) + (0.5,-0.4)$) {};
  %\draw [-latex,very thick] (d_v1_bottom.center) -- (d_v1_top.center);
  %\node[above=of d_v1_top, xshift=0cm, yshift=-1.35cm] (id_d_v1) {\protect\tikz[inner sep=.25ex,baseline=-.75ex] \protect\node[circle,draw] {{\tiny 2'}};};
  \node (d_v1_top) at ($(ui2)!0.5!(eq_vj1_vj2) + (1.5,0.25)$) {};
  \node (d_v1_bottom) at ($(ui2)!0.5!(eq_vj1_vj2) + (1.9,0.25)$) {};
  \draw [-latex,very thick] (d_v1_top.center) -- (d_v1_bottom.center);
  \node[right=of d_v1_top, xshift=-0.85cm, yshift=0cm] (id_f_u2) {\protect\tikz[inner sep=.25ex,baseline=-.75ex] \protect\node[circle,draw] {{\tiny 2'}};};
  
  % message from vj1 to delta
  \node (v1_d_top) at ($(vj1)!0.5!(eq_vj1_vj2) + (0.25,0.3)$) {};
  \node (v1_d_bottom) at ($(vj1)!0.5!(eq_vj1_vj2) + (0.25,-0.3)$) {};
  \draw [-latex,very thick] (v1_d_top.center) -- (v1_d_bottom.center);
  \node[below=of v1_d_bottom, xshift=0.3cm, yshift=1.75cm] (id_u1_d) {\protect\tikz[inner sep=.25ex,baseline=-.75ex] \protect\node[circle,draw] {{\tiny 4'}};};
  
  % Equality nodes for white text eq sign
  \node[latent, below=of ui1, draw=none, xshift=-0.025cm,yshift=.22cm,opacity=0, text opacity=1]  (eq)   {\textcolor{white}{\textbf{=}}};
  \node[latent, below=of vj1, draw=none, xshift=0cm,yshift=.22cm,opacity=0, text opacity=1]  (eq)   {\textcolor{white}{\,\textbf{=}}};
  \node[latent, right=of ui2, xshift=0.04cm, draw=none,,opacity=0, text opacity=1]  (eq)   {\textcolor{white}{\textbf{ }}};
    %\sigma^2_{\boldsymbol{v}_{2,j}}
\end{tikzpicture}
